Augmentation with Projection: Towards an Effective and Efficient Data Augmentation Paradigm for Distillation

Knowledge distillation is one of the primary methods of transferring knowledge from large to small models. However, it requires massive task-specific data, which may not be plausible in many real-world applications. Data augmentation methods such as representation interpolation, token replacement, or augmentation with models are applied to tackle this problem. However, these data augmentation methods either potentially cause shifts in decision boundaries (representation interpolation), are not expressive enough (token replacement), or introduce too much computational overhead (augmentation with models). To this end, we propose AugPro (Augmentation with Projection), an effective and efficient data augmentation method for distillation. Our method builds on top of representation interpolation augmentation methods to maintain the diversity of expressions and converts the augmented data to tokens to avoid shifting decision boundaries. It uses simple operations that come with little computational overhead. The results on multiple GLUE tasks show that our methods can improve distillation performance by a large margin at a low time cost. Codes are available at https://github.com/google-research/google-research/tree/master/augpro.

==> sections/4_theory.tex <==
\section{AugPro satisfies three requirements}
\label{Sec:theory}
Combining Section \ref{Sec:intuition} and Section \ref{Sec:method}, it is easy to know AugPro is expressive since it supports representation interpolation operations (Requirement (1)), avoid shifting decision boundaries since augmented data are in the format of tokens (first half of Requirement (2)), and brings little computational overhead (low complexity and paralleled computing). This section will prove that AugPro can explore more diversified new data.
% \ziqi{TODO:  make it consistent with intro. (content and notion)}
% \yuexin{One-sentence intuition. Illustration.}

% We construct some simple theoretical examples to demonstrate the intuition behind our new projection approach.
% As discussed in the introduction, the intuitions to make projections are two-fold.

% On the one hand, we know the datasets are drawn from a discrete set.
% Using data outside the discrete set is not necessarily beneficial or even harmful.
% Take a simple two-dimensional problem that has linear separability as an example.

% Let $\calX=\{x_1=(2,2),x_2=(2,-2),x_3=(-2,-2),x_4=(-2,2)\}$ be the universe of all data to learn, and $y=\{ y_1=1,y_2=1,y_3=-1,y_4=-1\}$ be the corresponding labels.
% Run the linear support vector machine (SVM) with a hard margin, i.e., solve the following optimization problem:
% \begin{align*}
%     \min_{\beta,b}\|\beta\|^2\\
%     \mathrm{s.t.} \quad y_i(\beta^\top x_i+b)\geq 1,\quad\forall i
% \end{align*}
% We get the solution
% $   \beta=(1/2,0),b=0. \qquad(*) $\yuexin{What does this (*) mean?}
% Suppose we get data $\{x_2,x_4\}$ as the training dataset and do the augmentation.
% If we simply use $\mix$ without projection, we get $x_{\mix}=(x_2+x_4)/2$ as the augmented data, whose label $y_{\mix}=\sign(\beta^\top x_{\mix}+b)=1$,\footnote{We treat $\sign(0)=1$ for simplicity.} where we use the solution $(*)$.
% Now run the linear SVM with $\{x_2,x_4,x_{\mix}\}$ with labels $\{y_2,y_4,y_{\mix}\}$, we get $\beta_{\mix}=(1/2,-1/2)$ and $b_{\mix}=1$.
% Nevertheless, $\sign(\beta_{\mix}^\top x_1+b_{\mix})\neq y_1$ and $\sign(\beta_{\mix}^\top x_3+b_{\mix})\neq y_3$.
% As a comparison, suppose we run $\mixp$ and get $x_{\mixp}=x_3$ and label $y_{\mixp}=y_3$, running SVM with $\{x_2,x_{\mixp},x_{4}\}$ and labels $\{y_2,y_{\mixp},y_{4}\}$ gets the solution $\beta_{\mixp}=\beta$ and $b_{\mixp}=b$, and can correctly classify $x_1$ and $x_3$.

% A similar situation arises in $\FGSM$ and $\FGSMP$.
% Consider the case when $x_{4}$ is the training data, and $\FGSM$ adds random noises to $x_{4}$ and gets $x_{\FGSM}=(7,2)$ whose label $y_{\FGSM}=\sign(\beta^\top x_{\FGSM}+b)=1$. Solving SVM with $\{x_4,x_{\FGSM}\}$ and $\{y_{4},y_{\FGSM}\}$ gets $\beta_{\FGSM}=(9/2,0)$ and $b_{\FGSM}=5/9$, which mistake the classification of $x_1$ and $x_2$.

% \subsection{Explore new data}
% On the other hand, projection can help the model learn the new data which is not in the original data set.
Suppose $\calX=\{-1,1\}^{2\log n}$ is the universe of all data with labels $\calY$ to learn, and $\calX_\train$ is the training data compositing of $n$ samples uniformly and independently drawn from $\calX$.

Suppose $n$ is even.
Let $x(j)$ be the $j$-th coordinate of vector $x$.
We construct $\calX_{\mixp}$ as follows:
Index the elements in $\calX_{\train}$ arbitrarily, and $x_i$ denotes the $i$-th element. 
For each positive integer $i\in[n/2]$, we construct an augmented data $z_i$ such that, for each coordinate $j\in [2\log n]$, $z_i(j)=x_{2i-1}(j)$ if $x_{2i-1}(j)=x_{2i}(j)$, otherwise $z_i(j)$ is uniformly chosen from $\{1,-1\}$.
We have the following claim:
\begin{claim}
\label{clm:mixp}
    % With probability at least $1-1/\poly(n)$, $\calX\subset \calX_{\mixp}$.
    One has 
    \begin{align*}
\lim_{n\to\infty}\E[|\calX_{\mixp}|/|\calX_\train|]=3/2,
    \end{align*}
    where the expectation is taken over the randomness of both $\calX_\train$ and $\calX_{\mixp}$, and $|\cdot|$ denotes the carnality after removing duplicate elements.
\end{claim}

% \daogao{Put prel and proofs into the appendix.}

As for constructing $\calX_{\FGSMP}$, for each $x_i\in\calX_\train$, we 
add Gaussian $\calN(0,4)$ to each coordinate of $x_i$, and then project back to $\calX$ to get $w_i$.

\begin{claim}
% With probability at least $1-1/\poly(n)$, $\calX\subset\calX_{\FGSMP}$.
One has
\begin{align*}
    \lim_{n\to \infty}\E[|\calX_{\FGSMP}|/|\calX_\train|]=2,
\end{align*}
where the expectation is taken over the randomness of both $\calX_\train$ and $\calX_{\FGSMP}$.
% , and $|\cdot|$ denotes the carnality after removing duplicate elements.
\end{claim}

Proves of both claims are straightforward probabilistic arguments with martingales and Freedman's inequality and can be found in Appendix \ref{app:proof1} and \ref{app:proof2}.

Now we show that AugPro satisfies all three requirements theoretically. We conduct experiments to empirically justify the effectiveness and efficiency of AugPro.
% linear classification model $y=\sign(\beta^\top x-b\geq 0)$, where $y\in\{-1,1\}$ is the label, $x\in\calX$ is a data, $\calX\subset \R^2$ is a finite set denoting the universe of all data and $\beta\in\R^d$ is the ground-true parameter.
